Depth Quality-Inspired Feature Manipulation for Efficient RGB-D Salient Object Detection

RGB-D salient object detection (SOD) recently has attracted increasing research interest by benefiting conventional RGB SOD with extra depth information. However, existing RGB-D SOD models often fail to perform well in terms of both efficiency and accuracy, which hinders their potential applications on mobile devices and real-world problems. An underlying challenge is that the model accuracy usually degrades when the model is simplified to have few parameters. To tackle this dilemma and also inspired by the fact that depth quality is a key factor influencing the accuracy, we propose a novel depth quality-inspired feature manipulation (DQFM) process, which is efficient itself and can serve as a gating mechanism for filtering depth features to greatly boost the accuracy. DQFM resorts to the alignment of low-level RGB and depth features, as well as holistic attention of the depth stream to explicitly control and enhance cross-modal fusion. We embed DQFM to obtain an efficient light-weight model called DFM-Net, where we also design a tailored depth backbone and a two-stage decoder for further efficiency consideration. Extensive experimental results demonstrate that our DFM-Net achieves state-of-the-art accuracy when comparing to existing non-efficient models, and meanwhile runs at 140ms on CPU (2.2$\times$ faster than the prior fastest efficient model) with only $\sim$8.5Mb model size (14.9% of the prior lightest). Our code will be available at https://github.com/zwbx/DFM-Net.

==> backup.tex <==

\begin{table*}[htbp]
	\centering
	\caption{Quantitative benchmark results. $\uparrow$/$\downarrow$ for a metric denotes that a larger/smaller value is better. Our results is bolded and the scores/numbers better than us is highlighted in \underline{underline}.} 
	%The best scores/numbers are highlighted in \textbf{bold}.}
	\label{tab:benchmark}
	\footnotesize
    %\scriptsize
    %\tiny
	\renewcommand{\arraystretch}{0.5}
	\renewcommand{\tabcolsep}{0.5mm}
	\begin{tabular}{lr|ccccccccccccc|c||cc|c}
		\hline\toprule
		&\multirow{3}{*}{Metric}\centering    &PCF & MMCI & CPFP & DMRA &D3Net   &JL-DCF &UCNet  &SSF  &S2MA &CoNet  &cmMS &DANet &ATSA  &\ourmodel$^{*}$ &A2dele &PGAR &\ourmodel  \\&    &\scriptsize CVPR18 &\scriptsize PR19 &\scriptsize CVPR19 &\scriptsize ICCV19 &\scriptsize TNNLS20   &\scriptsize CVPR20 &\scriptsize CVPR20   &\scriptsize CVPR20
		&\scriptsize CVPR20
		&\scriptsize ECCV20   &\scriptsize ECCV20
		&\scriptsize ECCV20 &\scriptsize ECCV20 & \scriptsize Ours &\scriptsize CVPR20&\scriptsize ECCV20 &\scriptsize Ours\\
		&     &\cite{PCF}&\cite{MMCI}&\cite{CPFP} &\cite{DRMA} &\cite{D3Net}   &\cite{JLDCF} &\cite{UCNet}  &\cite{SSF} &\cite{S2MA} &\cite{CoNet}	&\cite{cmMS} &\cite{DANet}  &\cite{ATSA}  &-&\cite{A2dele} &\cite{PGAR}&- \\
		\specialrule{0em}{1pt}{0pt}
		\hline\hline
		\specialrule{0em}{0pt}{1pt}

		%\multirow{4}{*}{\begin{sideways}\cite{ju2014depth}\end{sideways}}
\multirow{3}{*}{\begin{sideways}\textit{}\end{sideways}}

& Size~(Mb)$\downarrow$  &534	&930	&278	&228	&530	&520	&119		&125	&330	&167		&430	&102	&123  &\textbf{93} &57 &62	&\textbf{9}
\\


		& CPU~(ms)$\downarrow$  &35762	&46886	&16946	&1521	&851	&7588	&1011		&650	&1900	&667		&946	&1147	&1344  &\textbf{357}    &313    &755 &\textbf{140}
 \\
		& GPU~(FPS)$\uparrow$  &5	&8	&6	&13	&32	&9	&42	&21	&25	&36		&15	&32	&29  &\textbf{70} &\textbf{120}	&61 &64
 \\
	    \midrule
		\multirow{4}{*}{\begin{sideways}\textit{SIP}\end{sideways}}
		%\multirow{4}{*}{\begin{sideways}\cite{ju2014depth}\end{sideways}}
		& $S_{\alpha}\uparrow$ &0.842	&0.833	&0.850	&0.806	&0.860	&0.879 &0.875		&0.874	&0.878	&0.858		&0.867	&0.878	&0.864  &\textbf{0.885} &0.829	&0.875 &\textbf{0.883}
\\
		& $F_{\beta}^{\rm max}\uparrow$  &0.838	&0.818	&0.851	&0.821	&0.861	&0.885 &0.879		&0.880	&0.884	&0.867		&0.871	&0.884	&0.873  &\textbf{0.890} &0.834	&0.877&\textbf{0.887}
 \\
		& $E_{\xi}^{\rm max}\uparrow$     &0.901	&0.897	&0.903	&0.875	&0.909	&0.923 &0.919		&0.921	&0.920	&0.913		&0.091	&0.920	&0.911   &\textbf{0.926} &0.889	&0.914&\textbf{0.926}
  \\
		& $\mathcal{M}\downarrow$  &0.071	&0.086	&0.064	&0.085	&0.063	&0.051	&0.051	&0.053	&0.054	&0.063	&0.061	&0.054	&0.058  &\textbf{0.049} &0.070 &0.059&\textbf{0.051}
 \\
		\midrule
		\multirow{4}{*}{\begin{sideways}\textit{NLPR}\end{sideways}}
		%\multirow{4}{*}{\begin{sideways}\cite{peng2014rgbd}\end{sideways}}
		& $S_{\alpha}\uparrow$ &0.874	&0.856	&0.888	&0.899	&0.912	&0.925	&0.920		&0.914	&0.915	&0.908		&0.915	&0.915	&0.907  &\textbf{0.926} &0.890 &0.918	&\textbf{0.923}
 \\
		& $F_{\beta}^{\rm max}\uparrow$    &0.841	&0.815	&0.867	&0.879	&0.897	&\textbf{0.916} &0.903	&0.896	&0.902	&0.887		&0.896	&0.903	&0.876  &0.912 &0.875	&0.898 &\textbf{0.908}
 \\
		& $E_{\xi}^{\rm max}\uparrow$   &0.925	&0.913	&0.932	&0.947	&0.953	&\textbf{0.962} &0.956		&0.953	&0.950	&0.945		&0.949	&0.953	&0.945  &0.961 &0.937 &0.948	&\textbf{0.957}
 \\
		& $\mathcal{M}\downarrow$ &0.044	&0.059	&0.036	&0.031	&0.025	&\textbf{0.022}	&0.025	&0.026	&0.030  &0.031		&0.027	&0.029	&0.028  &0.024	&0.031&0.028&\textbf{0.026}
 \\
		\midrule
		\multirow{4}{*}{\begin{sideways}\textit{NJU2K}\end{sideways}}
		%\multirow{4}{*}{\begin{sideways}\cite{niu2012leveraging}\end{sideways}}
		& $S_{\alpha}\uparrow$&0.877	&0.858	&0.879	&0.886	&0.900	&0.903	&0.897		&0.899	&0.894	&0.895		&0.900	&0.891	&0.901  &\textbf{0.912}	&0.868&0.906 &\textbf{0.906}
 \\
		& $F_{\beta}^{\rm max}\uparrow$  &0.872	&0.852	&0.877	&0.886	&0.900	&0.903	&0.895		&0.896	&0.889	&0.892	 &0.897 &0.880	&0.893   &\textbf{0.913} &0.872 &0.905	&\textbf{0.910}
 \\
		& $E_{\xi}^{\rm max}\uparrow$&0.924	&0.915	&0.926	&0.927	&0.950	&0.944	&0.936		&0.935	&0.930	&0.937		&0.936	&0.932	&0.921  &\textbf{0.950} &0.914&0.940	&\textbf{0.947}
 \\
		& $\mathcal{M}\downarrow$    &0.059	&0.079	&0.053	&0.051	&0.041	&0.043	&0.043		&0.043	&0.053	&0.047		&0.044	&0.048 	&0.040 &\textbf{0.039} &0.052&0.045&\textbf{0.042}
 \\
		\midrule
		\multirow{4}{*}{\begin{sideways}\textit{RGBD135}\end{sideways}}
		%\multirow{4}{*}{\begin{sideways}\cite{cheng2014depth}\end{sideways}}
		& $S_{\alpha}\uparrow$  &0.842	&0.848	&0.872	&0.900	&0.898	&0.929	&0.934		&0.905	&\textbf{0.941}	&0.910		&0.932	&0.904	&0.907	 &0.938 &0.884&0.894&\textbf{0.931}
  \\
		& $F_{\beta}^{\rm max}\uparrow$  &0.804	&0.822	&0.846	&0.888	&0.885	&0.919	&0.930		&0.883	&\textbf{0.935}	&0.896		&0.922	&0.894	&0.885 &0.932 &0.873&0.879	&\textbf{0.922}
  \\
		& $E_{\xi}^{\rm max}\uparrow$  &0.893	&0.928	&0.923	&0.943	&0.946	&0.968	&\textbf{0.976}		&0.941	&{0.973}	&0.945		&0.970	&0.957	&0.952  &0.973	&0.920&0.929&\textbf{0.972}
\\
		& $\mathcal{M}\downarrow$  &0.049	&0.065	&0.038	&0.030	&0.031	&0.022	& 0.019		&0.025	&0.021	&0.029		&0.020	&0.029	&0.024  &\textbf{0.019} &0.030&0.032	&\textbf{0.021}
 \\
		\midrule
		\multirow{4}{*}{\begin{sideways}\textit{LFSD}\end{sideways}}
% 		\multirow{4}{*}{\begin{sideways}\cite{LFSD~\cite{LFSD}}\end{sideways}}
		& $S_{\alpha}\uparrow$ &0.786	&0.787	&0.828	&0.839	&0.825	&0.854	&0.864	&0.859	&0.837	&0.862	&0.849	&0.845	&0.865
		 &\textbf{0.870} &0.834 & 0.833 &\textbf{0.865}
\\
		& $F_{\beta}^{\rm max}\uparrow$   &0.775	&0.771	&0.826	&0.852	&0.810	&0.862	&0.864		&0.867 &0.835	&0.859		&\textbf{0.869}	&0.846	&0.862  &0.866&0.832&0.831&\textbf{0.864}
\\
		& $E_{\xi}^{\rm max}\uparrow$   &0.827	&0.839	&0.863	&0.893	&0.862	&0.893	&0.905		&0.900 &0.873	&\textbf{0.907}		&0.896	&0.886	&0.905 
		&0.903&0.874 &0.893&\textbf{0.903}
\\
		& $\mathcal{M}\downarrow$  &0.119	&0.132	&0.088	&0.083	&0.095	&0.078	&\textbf{0.066}	&\textbf{0.066}	&0.094	&0.071		&0.074	&0.083	&0.064  &0.068	&0.077&0.093&\textbf{0.072}
\\
		\midrule
		\multirow{4}{*}{\begin{sideways}\textit{STERE}\end{sideways}}
		%\multirow{4}{*}{\begin{sideways}\cite{fan2020rethinking}\end{sideways}}
		& $S_{\alpha}\uparrow$   &0.875	&0.873	&0.879	&0.835	&0.899	&0.905	&0.903		&0.893	&0.890	&0.908		&0.895	&0.892	&0.897	 &\textbf{0.908}&0.885 &\textbf{0.903}&0.898
 \\
		& $F_{\beta}^{\rm max}\uparrow$ &0.860	&0.863	&0.874	&0.847	&0.891	&0.901	&0.899		&0.890	&0.882	&0.904	&0.891	&0.881	&0.884  &\textbf{0.904}	&0.885&0.893&\textbf{0.893}
 \\
		& $E_{\xi}^{\rm max}\uparrow$  &0.925	&0.927	&0.925	&0.911	&0.938	&0.946	&0.944		&0.936	&0.932	&0.948		&0.937	&0.930	&0.921  &\textbf{0.948}	&0.935&0.936&\textbf{0.941}
\\
		& $\mathcal{M}\downarrow$   &0.064	&0.068	&0.051	&0.066	&0.046	&0.042	&\textbf{0.039}		&0.044	&0.051	&0.040		&0.042	&0.048	&0.039 	&0.040 &0.043 &\textbf{0.044}&0.045
\\
		\bottomrule
		\hline
	\end{tabular}
	\vspace{-8pt}
\end{table*}
